Causal Reasoning in the Presence of Latent Confounders via Neural ADMG Learning

Latent confounding has been a long-standing obstacle for causal reasoning from observational data. One popular approach is to model the data using acyclic directed mixed graphs (ADMGs), which describe ancestral relations between variables using directed and bidirected edges. However, existing methods using ADMGs are based on either linear functional assumptions or a discrete search that is complicated to use and lacks computational tractability for large datasets. In this work, we further extend the existing body of work and develop a novel gradient-based approach to learning an ADMG with non-linear functional relations from observational data. We first show that the presence of latent confounding is identifiable under the assumptions of bow-free ADMGs with non-linear additive noise models. With this insight, we propose a novel neural causal model based on autoregressive flows for ADMG learning. This not only enables us to determine complex causal structural relationships behind the data in the presence of latent confounding, but also estimate their functional relationships (hence treatment effects) simultaneously. We further validate our approach via experiments on both synthetic and real-world datasets, and demonstrate the competitive performance against relevant baselines.

==> matts_maths_commands.tex <==
\RequirePackage{amsmath,amsthm,amssymb,amsbsy,algorithmic,mathtools,xcolor}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


%Lowercase Bold Letters
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

%Lowercase Mathcal Letters
\newcommand{\mca}{\mathcal{a}}
\newcommand{\mcb}{\mathcal{b}}
\newcommand{\mcc}{\mathcal{c}}
\newcommand{\mcd}{\mathcal{d}}
\newcommand{\mce}{\mathcal{e}}
\newcommand{\mcf}{\mathcal{f}}
\newcommand{\mcg}{\mathcal{g}}
\newcommand{\mch}{\mathcal{h}}
\newcommand{\mci}{\mathcal{i}}
\newcommand{\mcj}{\mathcal{j}}
\newcommand{\mck}{\mathcal{k}}
\newcommand{\mcl}{\mathcal{l}}
\newcommand{\mcm}{\mathcal{m}}
\newcommand{\mcn}{\mathcal{n}}
\newcommand{\mco}{\mathcal{o}}
\newcommand{\mcp}{\mathcal{p}}
\newcommand{\mcq}{\mathcal{q}}
\newcommand{\mcr}{\mathcal{r}}
\newcommand{\mcs}{\mathcal{s}}
\newcommand{\mct}{\mathcal{t}}
\newcommand{\mcu}{\mathcal{u}}
\newcommand{\mcv}{\mathcal{v}}
\newcommand{\mcw}{\mathcal{w}}
\newcommand{\mcx}{\mathcal{x}}
\newcommand{\mcy}{\mathcal{y}}
\newcommand{\mcz}{\mathcal{z}}

%Lowercase mathbb letters
\newcommand{\mbba}{\mathbb{a}}
\newcommand{\mbbb}{\mathbb{b}}
\newcommand{\mbbc}{\mathbb{c}}
\newcommand{\mbbd}{\mathbb{d}}
\newcommand{\mbbe}{\mathbb{e}}
\newcommand{\mbbf}{\mathbb{f}}
\newcommand{\mbbg}{\mathbb{g}}
\newcommand{\mbbh}{\mathbb{h}}
\newcommand{\mbbi}{\mathbb{i}}
\newcommand{\mbbj}{\mathbb{j}}
\newcommand{\mbbk}{\mathbb{k}}
\newcommand{\mbbl}{\mathbb{l}}
\newcommand{\mbbm}{\mathbb{m}}
\newcommand{\mbbn}{\mathbb{n}}
\newcommand{\mbbo}{\mathbb{o}}
\newcommand{\mbbp}{\mathbb{p}}
\newcommand{\mbbq}{\mathbb{q}}
\newcommand{\mbbr}{\mathbb{r}}
\newcommand{\mbbs}{\mathbb{s}}
\newcommand{\mbbt}{\mathbb{t}}
\newcommand{\mbbu}{\mathbb{u}}
\newcommand{\mbbv}{\mathbb{v}}
\newcommand{\mbbw}{\mathbb{w}}
\newcommand{\mbbx}{\mathbb{x}}
\newcommand{\mbby}{\mathbb{y}}
\newcommand{\mbbz}{\mathbb{z}}

%Uppercase Bold Letters
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

%Uppercase Mathcal Letters
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}

%Uppercase mathbb letters
\newcommand{\mbbA}{\mathbb{A}}
\newcommand{\mbbB}{\mathbb{B}}
\newcommand{\mbbC}{\mathbb{C}}
\newcommand{\mbbD}{\mathbb{D}}
\newcommand{\mbbE}{\mathbb{E}}
\newcommand{\mbbF}{\mathbb{F}}
\newcommand{\mbbG}{\mathbb{G}}
\newcommand{\mbbH}{\mathbb{H}}
\newcommand{\mbbI}{\mathbb{I}}
\newcommand{\mbbJ}{\mathbb{J}}
\newcommand{\mbbK}{\mathbb{K}}
\newcommand{\mbbL}{\mathbb{L}}
\newcommand{\mbbM}{\mathbb{M}}
\newcommand{\mbbN}{\mathbb{N}}
\newcommand{\mbbO}{\mathbb{O}}
\newcommand{\mbbP}{\mathbb{P}}
\newcommand{\mbbQ}{\mathbb{Q}}
\newcommand{\mbbR}{\mathbb{R}}
\newcommand{\mbbS}{\mathbb{S}}
\newcommand{\mbbT}{\mathbb{T}}
\newcommand{\mbbU}{\mathbb{U}}
\newcommand{\mbbV}{\mathbb{V}}
\newcommand{\mbbW}{\mathbb{W}}
\newcommand{\mbbX}{\mathbb{X}}
\newcommand{\mbbY}{\mathbb{Y}}
\newcommand{\mbbZ}{\mathbb{Z}}




%Common domains, S,R,C,Z,N...
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}



%Theorem Environments

\newtheorem{prop}{Proposition}
\crefname{prop}{Proposition}{Propositions}
\newtheorem{miniprop}{Mini-Proposition}
\newtheorem{thm}{Theorem}
\crefname{thm}{Theorem}{Theorems}

\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\crefname{lem}{Lemma}{Lemmas}

\newtheorem{ex}{Example}
\newtheorem{rem}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{defi}{Definition}
\crefname{defi}{Definition}{Definitions}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}

\crefname{assumption}{Assumption}{Assumptions}
\Crefname{thm}{Theorem}{Theorems}
\Crefname{lem}{Lemma}{Lemmas}

\newenvironment{sproof}{%
  \renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

% \Crefname{prop}{Proposition}{Propositions}


%Commonly used matrices for GPs/Sparse Inference
\newcommand{\Kff}{\bfK_{\bf ff}}
\newcommand{\tilk}{\tilde{\bfK}_{\bf ff}}
\newcommand{\Qff}{\bfQ_{\bf ff}}
\newcommand{\KZ}{\bfK_{\bf Z}}
\newcommand{\Kuf}{\bfK_{\bf uf}}
\newcommand{\Kuu}{\bfK_{\bf uu}}



%miscellaneous
\def\*#1{\boldsymbol{\mathbf{#1}}}
\newcommand\ci{\perp\!\!\!\perp}

\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\Ahat}{\mathbf{\hat{A}}}
\newcommand{\Ghat}{\mathbf{\hat{G}}}
\newcommand{\Khat}{\mathbf{\hat{K}}}
\newcommand{\bfYp}{\mathbf{Y_{\bullet}}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\ddx}{\frac{d}{dx}}

\newcommand{\sn}{\sigma_{n}}

\newcommand{\mcLl}{\mathcal{L}_\text{lower}}
\newcommand{\mcLu}{\mathcal{L}_\text{upper}}
\newcommand{\dxdt}{\frac{\partial{x}}{\partial{t}}}
\newcommand{\dt}{\partial{t}}
\newcommand{\ddt}{\frac{\partial}{\partial{t}}}
\newcommand{\ddxd}{\frac{\partial}{\partial{x_d}}}
\newcommand{\ddxdp}{\frac{\partial}{\partial{x_{d'}}}}

\newcommand{\FT}{\frac{1}{\sqrt{2\pi}}\int g(x) e^{-i\omega x}dx}

\newcommand{\sgn}{\text{sgn}}

\newcommand{\transpose}{^\mathrm{\textsf{\tiny T}}}
\newcommand{\ExpSymb}{\mathbb{E}}
\newcommand{\Exp}[2]{\ExpSymb_{#1}\left[#2\right]}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\FromDist}{\sim}
\newcommand{\KL}[2]{\mathrm{KL}\left[ {#1} || {#2} \right]}
\newcommand{\KLint}[3]{\int #1 \log \left( \frac{#1}{#2} \right) \calcd{#3}}
\newcommand{\entropy}[1]{\mathcal{H}\left( #1 \right)}
\newcommand{\given}{\,\vert \,}
\newcommand{\quadform}[2]{{#2}\transpose{#1}{#2}}
\newcommand{\Normal}[3]{\mathcal{N}\left({#1}; {#2}, {#3}\right)}
\newcommand{\shortNormal}[2]{\mathcal{N}\left(#1, #2\right)}
\newcommand{\cov}{\text{cov}}

%comment in color
\RequirePackage{color}
\newcommand{\drb}[1]{{\color{red} (DRB: #1)}}
\newcommand{\aykf}[1]{{\color{blue} (AYKF: #1)}}

\newcommand{\outline}[1]{{\color{purple} Outline Notes: #1}}

\newcommand\aseq{\stackrel{\mathclap{\scriptstyle{a.s.}}}{=}}

\newcommand{\bfLam}{\mathbf{\Lambda}}

\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\mathdash}{\relbar\mkern-9mu\relbar}
